Prior Flow Variational Autoencoder: A density estimation model for Non-Intrusive Load Monitoring

Non-Intrusive Load Monitoring (NILM) is a computational technique to estimate the power loads' appliance-by-appliance from the whole consumption measured by a single meter. In this paper, we propose a conditional density estimation model, based on deep neural networks, that joins a Conditional Variational Autoencoder with a Conditional Invertible Normalizing Flow model to estimate the individual appliance's power demand. The resulting model is called Prior Flow Variational Autoencoder or, for simplicity PFVAE. Thus, instead of having one model per appliance, the resulting model is responsible for estimating the power demand, appliance-by-appliance, at once. We train and evaluate our proposed model in a publicly available dataset composed of power demand measures from a poultry feed factory located in Brazil. The proposed model's quality is evaluated by comparing the obtained normalized disaggregation error (NDE) and signal aggregated error (SAE) with the previous work values on the same dataset. Our proposal achieves highly competitive results, and for six of the eight machines belonging to the dataset, we observe consistent improvements that go from 28% up to 81% in NDE and from 27% up to 86% in SAE.

==> content/acknowledgment.tex <==
% \section*{Acknowledgment}
This material is based upon work supported by Air Force Office Scientific Research under award number FA9550-19-1-0020.
Also, this study was financed in part by the Coordenação de Aperfeiçoamento de Pessoal de Nível Superior – Brasil (CAPES) – Finance Code 001.

==> content/architecture-details/old/CNF_Network.tex <==
%%\subsubsection*{CNF Network}
    The CNF network is an invertible conditional normalizing flow model 
        mainly inspired by the Glow \cite{Kingma2018GlowGF} architecture.
    This network is responsible for learning the latent space prior distribution $\pi(z_{0}|y)$ given the observations $y$.
    
    The CNF network consists of {\NCNFBlocks} stacked step-flow blocks \cite{Kingma2018GlowGF}, 
        which, in it turns, 
        is a stacking of 
        an Actnorm layer, 
        an Invertible $1 \times 1$ Convolution layer, 
        and an Affine Coupling layer.
    
    At each block, 
    the Invertible $1 \times 1$ Convolution outputs are given as inputs to the Affine Coupling Layer.
    % The affine coupling layers receives as inputs the outputs of the Invertible $1 \times 1$ Convolution.
    Subsequently, 
        as described in Section \ref{sec:conditional-flow},
        the inputs are split into two halves. 
    The first half is then concatenated with the conditioning network outputs before calculating operators 
        $s$ and $t$.
    Those operators ($s$ and $t$) are calculated by a backbone network, 
        a standard neural network block illustrated in Figure \ref{fig:s-and-t-block}.
        \begin{figure}[H]
            \centering
            \includegraphics[width=\linewidth]{content/architecture-optimization/images/s-t-block-v2.png}
            \caption{Coupling Layer's backbone}
            \label{fig:s-and-t-block}
        \end{figure}
    % The backbone is composed of a sequence of stacked 
    %     convolution, Layer Normalization layers \cite{Ba2016LayerN},
    %     and Relu activation function. 
    % All Convolutional layers in the backbone have {\CNFConvFilters} filters of size {\CNFkernelSize},
    %     except for the last convolution,
    %     which has {\Zsize} filters.
        % which the number of filters is set such that the backbone inputs 
        % and outputs 
        % are equal-sized.
    
    
    % In section \ref{sec:conditional-flow}, 
    %     we also mentioned that the model learns the prior distribution parameters
    %     $\mu_{z_{k}}$ and $\sigma^{2}_{{z_{k}}}$.
    % In practice, 
    %     those parameters are the outputs of two convolutional layers that receive as inputs the conditioning network outputs $h(y)$.
    % The first $\mu_{z_{k}}(h(y))$ has {\Zsize} filters of size {\EncoderLastKSize} and no activation function.
    % The second $\sigma^{2}_{z_{k}}(h(y))$ has {\Zsize} filters of size {\EncoderLastKSize} and uses the sigmoid as its activation function.

==> content/architecture-details/old/decoder_network.tex <==
%%\subsubsection*{Decoder Network}

    The Decoder network is a straightforward conventional neural network 
        responsible for decoding the examples from the latent space $z_{0}$ back to the observation space $x$.
    In other words, 
        the Decoder Network decodes the latent representations $z_{0}$ 
        into an estimate for each appliance's individual active power demand.
        
    Thus, 
        the Decoder Network is composed of {\NDecoderBlocks} decoder blocks followed by two simple convolutional layers.
    \begin{figure}[ht!]
        \centering
        \begin{tikzcd}
            \text{Gated Convolution} \arrow{r} &%\\%& 
            \text{Transposed Gated Convolution}
        \end{tikzcd}
        \caption{Decoder block.}
        \label{fig:decoder-block}
    \end{figure}
    The decoder block is illustrated in Figure \ref{fig:decoder-block}
        and is composed of a gated convolution layer 
        and a transposed gated convolution layer \cite{Berg2018SylvesterNF}.
    The transposed gated convolution doubles the temporal dimension at each block.
    % The temporal dimension is doubled by the transposed gated convolution at each block.
    Both layers have {\DecoderFilters} filters of size {\DecoderKSize}.
    After being passed through the {\NDecoderBlocks} decoder blocks, 
        the inputs are passed through two additional convolutional layers.
    The first has {\DecoderFilters} filters of size {\DecoderKSize},
        and the second has as many filters as the number of individual appliances being estimated by the model.
    Both layers have stride $1$ and no activation function.

==> content/architecture-details/old/encoder_and_conditioning_networks.tex <==
%%\subsubsection{Encoder Network and Conditioning Network}
    The encoder network is a simple full gated convolutional neural network \cite{Dauphin2017LanguageMW}.
    It receives the concatenated vectors $[x;y]$ as inputs
        and then encodes them into a latent representation $z_{0}$.
    % In other words, 
    %     it receives a concatenation of the aggregated power demand features $y$ 
    %     with the individual appliances' active power $x$
    %     and then encodes it into the latent space $z_{0}$.
    % Thus, 
    %     the encoder network learns a mapping $f: x,y \rightarrow z_{0}$, 
    %     where $z_{0}$ follows the posterior distribution.
    
    % Similarly,
    The conditioning network is also a full gated convolutional neural network 
        similar to the encoder network.
    The encoder and conditioning network diverges only in the last layers and outputs.
    % The encoder and conditioning network diverges only in that
    %     the encoder has one additional simple convolutional layer on its top.
    Therefore the conditioning network receives the data $y$,
        encodes it into a rich representation $h(y)$
        and into the base distribution $\pi(z_{k}|y)$ parameters $\mu(h(y))$ and $\sigma(h(y))$.
        
    Those networks are composed of {\NEncoderBlocks} blocks 
        built by stacking two gated convolutional layers \cite{Berg2018SylvesterNF}.
    Figure \ref{fig:encoder-block} illustrates the encoder block.
    \begin{figure}[ht!]
        \centering
        \begin{tikzcd}
            \text{Gated Convolution} \arrow{r} &%\\%& 
            \text{Gated Convolution}
        \end{tikzcd}
        \caption{Encoder block.}
        \label{fig:encoder-block}
    \end{figure}
    At each block, 
        the input's temporal dimension is halved by the second gated convolutional layer, 
        which has strides equals $2$, 
        in contrast to the first layer
        with strides equal to $1$.
    Additionally,
        both gated convolutional layers have {\EncoderFilters} filters of size {\EncoderKSize}.
    Subsequently, 
        after {\NEncoderBlocks} blocks, both
        the encoder 
        and the conditioning networks 
        have an additional gated convolutional layer 
        with {\EncoderFilters} filters of size {\EncoderKSize}. 
    
    The encoder network has one additional convolutional layer 
        that receives the last Gated Convolution outputs as its inputs, 
        outputting $z_{0}$.
    This convolutional layer has 
        {\Zsize} filters 
        of size {\EncoderLastKSize} 
        and stride $1$.
    
    In its turn, 
        the conditioning network has two additional convolutional layers which 
        both receive the outputs $h(y)$ of the last Gated Convolution as its inputs, 
        outputting $\mu(h(y))$ and $\sigma(h(y))$.
    These convolutional layers have 
        {\Zsize} filters 
        of size {\EncoderLastKSize} 
        and stride $1$.
    Additionally, 
        the convolutional layer that outputs $\sigma(h(y))$ uses the sigmoid as its activation function.

==> content/background/equations/eq_change_of_variable_formula.tex <==
\begin{equation}
    \label{eq:change-of-variable-formula}
    p(x) = \pi_{Z}(f_{\omega}(x)) 
        \left | 
            det 
            \left (
                    \frac
                        { \partial f_{\omega}(x) }
                        {\partial x} 
                \right ) 
            \right |
\end{equation}

==> content/background/equations/eq_change_of_variable_formula_conditional.tex <==
\begin{equation}
    \label{eq:conditional-change-of-variable-formula}
    p(x) = \pi(f_{\omega}(x,y)|y)\left | det \left (\frac{\partial f_{\omega}(x,y)}{\partial x} \right ) \right |
\end{equation}

==> content/background/equations/eq_elbo.tex <==
\begin{equation}
    \label{eq:elbo}
    log\ p_{\theta}(x) \geq \mathbb{E}_{q} \left [\ log\ p_{\theta}(x|z)\ \right ] - \mathbb{KL}(q(z|x) || p(z)) 
\end{equation}
% In such a model, 
%     $x$ is generated by sampling from the estimated distribution $p_{\theta}(x|z)$, 
%     which is conditioned on the unobserved latent variable $z$.
%     where $\theta$ represents the neural network parameters that are learned by maximizing the lower bound defined by ELBO \ref{eq:elbo}.
    % conditioned on an unobserved latent variable $z$
    
% Moreover,
%     the posterior approximation $q_{\phi}(z|x)$ addresses the intractability of the true posterior
%     and is also done by a neural network.
    % which predicts the distribution's variational parameters.

==> content/background/equations/eq_elbo_cvae.tex <==
\begin{equation}
    \label{eq:elbo-cvae}
    log\ p_{\theta}(x|y) \geq \mathbb{E}_{q} \left [\ log\ p_{\theta}(x|z,y)\ \right ] - \mathbb{KL}(q(z|x,y) || \pi(z|y)) 
\end{equation}

==> content/background/invertible_layers/actnorm.tex <==
\subsubsection{ActNorm}
    Also introduced by the Glow model \cite{Kingma2018GlowGF},
        the ActNorm layer is proposed, 
        as an alternative to the standard batch normalization \cite{Ioffe2015BatchNA},
        for models trained with small mini-batches.
    Similar to the batch normalization, 
        the ActNorm layer performs a per-channel normalization in the network activations.
    Thus,
        the ActNorm layer performs an affine transformation to shift 
        and scale the network activations, 
        using its scale 
        and bias trainable parameters.
    
    Additionally, 
        the scale and bias parameters are initialized such that 
        the activations after the Actnorm layer have approximately zero mean 
        and unit variance.
    
    Finally, 
        the log-determinant is computed as follows:
        \begin{equation}
            \label{eq:acnorm-logdet}
            log \left | det\left ( \frac{ \partial s \odot x + b}{\partial x} \right ) \right | = w \cdot sum(log|s|)
        \end{equation}
    In equation \ref{eq:acnorm-logdet},
        $x$ is the layer input, 
        $s$ is the scale parameter, 
        $b$ is the bias parameter, 
        $\odot$ is an element-wise product operation, 
        and $w$ stands for the input width dimensions.


==> content/background/invertible_layers/coupling-layers.tex <==
\subsubsection{Affine Coupling Layers}
    
    The affine coupling layer, 
        first introduced in Nice and RealNVP \cite{Dinh2014NICENI, Dinh2016DensityEU},
        is a simple bijective layer that is simple to invert 
        and has a tractable Jacobian determinant. 
    In this layer,
        the input vector is partitioned into two halves, 
        and then one partition is updated using complex dependencies computed from the other partition.
    In the end, 
        the layer concatenates the partitions into a vector containing the same dimensions as its input. 
    Thus, 
        given $D$-dimensional input $x$ and a scalar $d < D$, 
        the affine coupling layer output $h$ follows:
            \begin{equation}
                \label{eq:affine-coupling-layer}
                h = 
                \left\{
                \begin{matrix}
                    h_{1:d} = x_{1:d}; \\ 
                    h_{d+1:D} = x_{d+1:D} \odot  exp(s(x_1:d)) + t(x_{1:d})
                \end{matrix}
                \right.
            \end{equation}
        where $s$ and $t$ 
        are functions from $\mathcal{R}^{d} \rightarrow \mathcal{R}^{D - d}$, 
        and $\odot $ is the element-wise product.
    
    The Jacobian of the transformation expressed in equation \ref{eq:affine-coupling-layer}, 
        is as follows:
            \begin{equation}
                \label{eq:affine-coupling-jacobian}
                J =  
                \begin{bmatrix}
                    \mathbb{I}_{d} & 0_{d\times(D-d)} \\ 
                    \frac{\partial h_{d+1:D}}{\partial x_{1:d}} & diag(exp(s(x_{1:d})))
                \end{bmatrix}
            \end{equation}
    In equation \ref{eq:affine-coupling-jacobian}, 
        $diag(exp(s(x_{1:d})))$ 
        is the diagonal matrix whose diagonal elements correspond to the vector 
        $s(x_{1:d}))$. 
    Since the Jacobian is upper triangular, 
        its determinant is efficiently computed as 
        $exp \left[ \sum_{j} s( x_{1:d})_{j} \right ]$.
    
    Since computing the Jacobian determinant of the affine coupling layer does not involve calculating the $s$ and $t$ Jacobians, 
        those operators are calculated by a standard neural network block that serves as the layer's backbone.
    
    Finally, 
        computing the inverse of the coupling layer is no more complex than the forward propagation, 
        and therefore, 
        sampling is as efficient as inference. 
    Equation \ref{eq:affine-coupling-layer-inverse} defines the inverse transformation of the affine coupling layer.
        \begin{equation}
            \label{eq:affine-coupling-layer-inverse}
            x = 
            \left\{
            \begin{matrix}
                x_{1:d} = h_{1:d}; \\ 
                x_{d+1:D} = (h_{d+1:D} - t(h_{1:d})) \odot  exp(-s(h_{1:d}))
            \end{matrix}
            \right.
        \end{equation}
    
    % \subsubsection*{Split and concatenation}
    % The affine coupling layer splits the input tensor $x$ into two halves, 
    %     and at the end, 
    %     the layer undoes the split by concatenating the two halves into a single tensor again.

==> content/background/invertible_layers/invertible-conv.tex <==
\subsubsection{Invertible 1 x 1 convolutions}

    The Glow model architecture \cite{Kingma2018GlowGF} proposes to replace the most commonly used fixed permutations \cite{Dinh2014NICENI, Dinh2016DensityEU} operator with a $1 \times 1$ invertible convolutional layer,
        which they claim to be a generalization of the permutation operators.
    
    In this layer,
        the convolution weight matrix is initialized as a random rotation matrix, with the same number of filters as the number of input channels $c$.
        % and the number of channels $c$ in its 
        % inputs and outputs is the same. 
        % reescrive assim ^ o que vc acha?
        
    Thus, 
        the invertible $1 \times 1$ convolution receives a tensor 
        $x \in \mathbb{R}^{w \times c}$ 
        as input and applies the convolutional operator using the weight matrix 
        $W \in \mathbb{R}^{c \times c}$ as its convolutional kernel.
    Additionally,  
        the weight matrix $W$ is initialized such that its initial log-determinant is $0$.
    
    Finally, 
        the log-determinant of this layer is computed as follows:
            \begin{equation}
                \label{eq:inv-conv-logdet}
                log \left | det\left ( \frac{\partial conv2D(h; W)}{\partial h} \right ) \right | = width \cdot log|det(W)|
            \end{equation}

        
    
    
   

==> content/background/old/background.tex <==
\section{Background} \label{sec:background}

    This section discusses recent efforts in Variational Autoencoders (VAEs); 
    Invertible Normalizing Flows(NF);
    and their conditional case extensions.
    
    \input{content/background/vae}
    \input{content/background/cvae}
    \input{content/background/normalizing_flows}
    \input{content/background/conditional_flow}

==> content/background/old/conditional_flow.tex <==
\subsection{Conditional Normalizing Flow Models} \label{sec:conditional-flow}

    The Conditional Normalizing Flow (CNF) is an NF extension to the conditional case.
    Thus,
        CNF extends the NF by conditioning the entire generative process on an input $y$ \cite{Ardizzone2019GuidedIG, Winkler2019LearningLW}.
    
    The goal is to learn conditional likelihoods using conditional normalizing flows for complicated target distributions in multivariate prediction tasks.
    
    Given an input $y$ and a target $x$,
        we learn the distribution $p(x|y)$ 
        using the conditional base distribution $\pi(z_{k}|y)$ 
        and a sequence of $k$ mappings 
        $$
            z_{k} = f_{\omega}(x,y) = f^{k}(...(f^{1}(x,y),y),y)
        $$
        % $f_{i}: X \times Y \rightarrow Z$, 
        which are bijective in $x$ 
        and $z_{k}$.
    Thus,
        the change of variables formula becomes:
            \begin{equation}
                \label{eq:conditional-change-of-variable-formula}
                p(x|y) = \pi(f_{\omega}(x,y)|y)\left | det \left (\frac{\partial f_{\omega}(x,y)}{\partial x} \right ) \right |
            \end{equation}
    % The bijective mapping $f_{\omega}$ allows modelling multimodal distributions \cite{Winkler2019LearningLW}.
    
    The generative process is done by 
        first sampling $z_{k}$ from a simple base density,
        which has its parameters determined by an arbitrary function that receives $y$ as input. % (for us this is a diagonal Gaussian) 
    Then, 
        $z_{k}$ is transformed by the sequence of bijective mappings $f^{-1}_{\omega}(z_{k}, y)$. 
    Therefore, 
        the generative process is defined as:
            \begin{equation}
                \label{eq:z-follows-p}
                z_{k} \sim \pi(f_{\omega}(x,y)|y)
            \end{equation}
            \begin{equation}
                \label{eq:x-fz}
                x = f_{\omega}^{-1}(z_{k},y)
            \end{equation}

    During the training procedure,
        $x$ and $y$ are given as inputs to the model 
        and passed through the invertible mapping $f_{\omega}(x,y)$ 
        to yield $z$.
    Then the base distribution parameters and the log-likelihood are evaluated.
    As usual, 
        in neural networks, 
        the flow and base distribution parameters are optimized using stochastic gradient descent with mini-batches. 
    
    %%In our work, 
    % The conditioning is introduced in the prior distribution.
    
    %     the prior parameters (mean and variance) are defined by arbitrary functions such that: 
    %     % we set the mean and variance as functions of $y$ such that
    %     \begin{equation}
    %         \label{eq:prior-net}
    %         \pi(z_{k}|y) = \mathcal{N}(z; \mu(y), \sigma^{2}(y)),
    %     \end{equation}
    %     where $\mu(y)$ and $\sigma^{2}(y)$ are the outputs of a standard neural network.
    The conditioning is introduced  
        (I) in the affine coupling layer
        and (II) in the prior. 
    For the affine coupling layers,
    % In it turns, 
        we pass the conditional information as input to the internal layer's operators, such as proposed by Ardizzone \cite{Ardizzone2019GuidedIG}. %%$s$ and $t$.
    So,
        the forward pass of the affine coupling layer becomes:
        \begin{equation}
            \label{eq:cond-affine-coupling-layer}
            z =
            \left \{
            \begin{matrix}
                z_{1:d} = x_{1:d}; \\ 
                z_{d+1:D} = x_{d+1:D} \odot  e^{s([x_{1:d}; h(y)])} + t([x_{1:d}; h(y)])
            \end{matrix}
            \right.
        \end{equation}
        where $[\cdot; \cdot]$ represents a concatenation, 
        $x = [x_{1:d}; x_{d+1:D}]$,
        and $z = [z_{1:d}; z_{d+1:D}]$ is the layer output.
    Moreover,
        the conditioning term is the output of a network that transforms the input $y$ into a rich representation $h(y)$.
    % In practice,
    %     the conditioning term $y$ is transformed by network $h(y)$ into a rich representation before being passed to the layer.
    % Thus,
    %     each coupling layer's $s$ and $t$ operators are applied to 
    %     the concatenation $[x_{1:d}; h(y)]$.
    
    Finally,
    % In it turns, 
    % For the prior, 
        the base distribution parameters are set by arbitrary functions such that:
        % we set the mean and variance as functions of $y$ such that
        \begin{equation}
            \label{eq:prior-net}
            \pi(z_{k}|y) = \mathcal{N}(z; \mu(h(y)), \sigma(h(y))),
        \end{equation}
        where $\mu(h(y))$ and $\sigma(h(y))$ are the outputs of a standard neural network that uses the conditioning term $h(y)$ as input.
        
    


==> content/background/old/cvae.tex <==
\subsection{Conditional Variational Autoencoders} \label{sec:cvae}

    The Conditional Variational Autoencoder (CVAE) is a VAE extension to the conditional case.
    Thus,
        CVAE extends the VAE's math by conditioning the entire generative process on an input $y$ \cite{Sohn2015LearningSO, Walker2016AnUF}.
    Such a model allows us to tackle problems where 
        the input-to-output mapping is one-to-many
        without requiring the output distribution structure specification \cite{Doersch2016TutorialOV}.   
        % us to explicitly specify the structure of the output distribution \cite{Doersch2016TutorialOV}.
    
    Given an input $y$ and an output $x$, 
        CVAE aims at creating a model $p( x | y )$, 
        which maximizes the probability of ground truth.
        % which maximizes the ground truth's probability. 
    The model is defined by introducing a latent variable 
        $z \sim \mathbb{N}( 0, I )$, 
        such that:
        \begin{equation}
            \label{eq:elbo-cvae}
            log\ p_{\theta}(x|y) \geq \mathbb{E}_{q} \left [\ log\ p_{\theta}(x|z,y)\ \right ] - \mathbb{KL}(q_{\phi}(z|x,y) || \pi(z|y)) 
        \end{equation}
    
    % During training, 
    %     the posterior distribution model $q_{\phi}(z|x, y)$ 
    %     and the data distribution model $p_{\theta}( x | z, y)$
    %     are learned by neural networks with 
    %     $\phi$ and $\theta$ parameters.

    At inference time, 
        we sample from the distribution $p( x | y )$ by simply sampling $z$ from the prior distribution $\pi( z | y ) = \mathbb{N}( 0, I )$. %,
        % which still is $\mathbb{N}( 0, I )$.
    Thus, at inference time, 
        $z$ is sampled independently from $y$.

==> content/background/old/normalizing_flows.tex <==
\subsection{Normalizing Flow Models} \label{sec:normflow}
    
    Normalizing Flow (NF) models 
    \cite{Dinh2014NICENI, Dinh2016DensityEU, Kingma2018GlowGF} 
        learn flexible posteriors by transforming a simple base distribution with a sequence of invertible transformations, 
        known as normalizing flows. 

    Given two vector-spaces $X \in R^{d}$ and $Z \in R^{d}$,
        an invertible mapping $f_{\omega}: X \rightarrow Z$,
        a base distribution $\pi(z)$,
        and parameters $\omega$,
        then normalizing flows compute the data log-likelihood 
            $log\ p(x)$ using the change of variables formula:
            % $log\ \pi_{X}(x)$ 
            \begin{equation}
                \label{eq:change-of-variable-formula}
                p(x) = \pi(f_{\omega}(x)) 
                    \left | 
                        det 
                        \left (
                                \frac
                                    { \partial f_{\omega}(x) }
                                    {\partial x} 
                            \right ) 
                        \right |
            \end{equation}
    In equation \ref{eq:change-of-variable-formula}, 
        the term $| det( \partial f_{\omega}(x)/ \partial x ) |$
        is the Jacobian Determinant absolute value,
        or for simplicity, the Jacobian of $f_{\omega}$.
    It measures the change in density when going from $x$ to $z$ under the transformation $f_{\omega}$.
    In general, 
        the cost of computing the Jacobian will be $O(D^{3})$.
    However,
        it is possible to design transformations in which the Jacobians are efficiently calculated \cite{Kingma2018GlowGF}.
        
    The main challenge in invertible normalizing flows \cite{Winkler2019LearningLW} is to design mappings to compose the transformation $f_{\omega}$ since they must have a set of restricting properties. 
    Thus,
        all mappings $f^{i} \in f_{\omega}$ must have 
        a known and tractable inverse mapping  
        and an efficiently computable Jacobian,
        while being powerful enough to model complex transformations.
    Moreover, 
        fast sampling is desired, 
        so the inverse mappings $(f^{i})^{-1}$ should be calculated efficiently. 
    
    Fortunately, 
        there is a set of well-established invertible layers with all those properties in the current literature of normalizing flows.
    This work is built upon three of them 
    \footnote{Due to space constraints we refer to \cite{Kingma2018GlowGF} for more details on those invertible layers.}: 
            (I) the Affine Coupling layer 
            \cite{Dinh2014NICENI, Dinh2016DensityEU};  
            (II) the Invertible $1\times1$ Convolution layer \cite{Kingma2018GlowGF}; 
            (III) the Actnorm layer \cite{Kingma2018GlowGF}.
    
    % In the following, 
    %     we present the invertible layers that we use in this work.
    
    % \input{content/background/invertible_layers/coupling-layers}
    % \input{content/background/invertible_layers/invertible-conv}
    % \input{content/background/invertible_layers/actnorm}
    % TODO: stepflow block


==> content/background/old/vae.tex <==
\subsection{Variational Autoencoder} \label{sec:vae}

    Consider a probabilistic model $p_{\theta}(x, z)$ with observations $x$, 
        continuous latent variables $z$,
        and model parameters $\theta$. 
    In generative modeling, 
        we are often interested in learning the model parameters $\theta$ by estimating the marginal likelihood $p_{\theta}(x)$.  
    Unfortunately,
        the marginalization over the unobserved latent variables $z$ is generally intractable \cite{Kingma2013AutoEncodingVB}.  
    
    Instead,
        variational inference \cite{Jordan1999AnIT}  constructs a lower bound 
        on the marginal likelihood logarithm  $log\ p_{\theta}(x)$. 
    The lower bound is built by introducing a variational approximation to the posterior.
        % $q_{\phi}(z|x)$ to the posterior.
        \begin{equation}
            \label{eq:elbo}
            log\ p_{\theta}(x) \geq \mathbb{E}_{q} \left [\ log\ p_{\theta}(x|z)\ \right ] - \mathbb{KL}(q_{\phi}(z|x) || \pi(z)) 
        \end{equation}
    Equation \ref{eq:elbo} is called as 
        the Evidence Lower Bound (ELBO), 
        where $q_{\phi}(z|x)$ is the posterior approximation,
        $p_{\theta}(x|z)$ is a likelihood function,
        $\pi(z)$ is the prior distribution,
        and $\phi$ and $\theta$ are the model parameters.
    
    Thus,
        VAEs \cite{Kingma2013AutoEncodingVB} are generative models 
        that use neural networks 
        to predict the variational distribution parameters.
    The model parameters
        $\theta$ and $\phi$ are jointly trained through stochastic maximization of ELBO through the reparameterization trick \cite{Kingma2013AutoEncodingVB, Rezende2014StochasticBA}.


    It is worth mentioning that the better the posterior approximation, 
        the tighter the ELBO is, 
        and so smaller is the gap between the true distribution $p(x)$ and its lower-bound.
    However, 
        a diagonal-covariance Gaussian is usually chosen as the variational distribution $q_{\phi}(z|x)$.
    With such a simple distribution, 
        the ELBO will be fairly loose,
        resulting in biased maximum likelihood estimates \cite{Berg2018SylvesterNF}. %*of the model parameters  
    Therefore,  
        a more flexible posterior distribution is needed.

==> content/cfvae/equations/eq_cfvae_elbo.tex <==
% \begin{equation}
%     \label{eq:elbo-cfvae}
%     \begin{split}
%     log\ p_{\theta}(x|y) 
%     &\geq 
%         \mathbb{E}_{q} \left [\ log\ p_{\theta}(x|z_{0},y)\ \right ] 
%         - \mathbb{KL}(q_{\phi}(z_{0}|x,y) || \pi_{\omega}(z_{0}|y)) \\
%     &\geq 
%         \mathbb{E}_{q} \left [\ log\ p_{\theta}(x|z_{0},y)\ \right ]
%         - \mathbb{E}_{q_{\phi}(z_{0}|x,y)} \left [\ log\ q_{\phi}(z_{0}|x,y)\ \right ]
%         + \mathbb{E}_{q_{\phi}(z_{0}|x,y)} \left [\ log\ \pi_{\omega}(z_{0}|y)\ \right ]
%     \end{split}
% \end{equation}
\begin{multline}
    \label{eq:elbo-cfvae}
    % \begin{split}
    log\ p_{\theta}(x|y) \\ 
    % \geq
    %     \mathbb{E} \left [\ log\ p_{\theta}(x|z_{0},y)\ \right ] 
    %     - \mathbb{KL}(q_{\phi}(z_{0}|x,y) || \pi_{\omega}(z_{0}|y)) \\
    \geq 
        \mathbb{E} \left [\ log\ p_{\theta}(x|z_{0},y)\ \right ]
        - \mathbb{E} \left [\ log\ q_{\phi}(z_{0}|x,y)\ \right ]\\
        + \mathbb{E} \left [\ log\ \pi_{\omega}(z_{0}|y)\ \right ]
    % \end{split}
\end{multline}

==> content/cfvae/equations/eq_cfvae_loss.tex <==
\begin{equation}
    \label{eq:loss-elbo}
     \mathcal{L} = 
        -\mathbb{E} \left [\ log\ p_{\theta}(x|z_{0},y)\ \right ]
        - \mathbb{E} \left [\ log\ \pi_{\omega}(z_{0}|y)\ \right ]
\end{equation}%
%

==> content/cfvae/old/cfvae.tex <==
\section{\ModelFullName} \label{sec:pfvae}
    
    In this section, 
        we describe our proposed {\ModelName} model. 
    Our approach is to model NILM to estimate a noisy distribution 
        which is conditioned on the aggregated power demand.
    For this purpose, 
        we denote the aggregate data as $y$ 
        and the individual appliances data as $x$. 
        
    
    Inspired by ideas found in \cite{Berg2018SylvesterNF}, 
        we propose a formulation for Conditional Density Estimation (CDE),
        which joins CVAEs 
        \cite{Kingma2013AutoEncodingVB, Sohn2015LearningSO} 
        with invertible normalizing flows 
        \cite{Dinh2014NICENI, Dinh2016DensityEU, Kingma2018GlowGF} 
        to estimate the conditional power demand density for each appliance.
    The resulting {\ModelName} model is a CVAE extension 
        that uses a CNF model to learn the prior distribution $\pi(z_{0}|y)$. 
        % which makes the posterior approximation more flexible \cite{Sylvester}.
    Therefore, 
        {\ModelName} is divided into two components. 
    The first component is the CVAE that still learns 
        an inference $q_{\phi}(z_{0} | x,y)$ 
        and a generative $p_{\theta}(x | z_{0}, y)$ models. 
    The second component is a CNF model responsible for learning the prior distribution $\pi(z_{0} | y)$.
    % Therefore,
    %     the model still learns an inference $q_{\phi}(z_{0} | x,y)$
    %     and a generative $p_{\theta}(x | z_{0}, y)$ models in the CVAE part.  
    % The CNF part, in its turn, is responsible for learning the prior distribution $\pi(z_{0} | y)$.
    
    During the training procedure,
        the inference model outputs $z_{0}$.
    After that, 
        $z_{0}$ is passed throughout the CNF model, 
        which encodes $z_{0}$ into $z_{k}$.  
    % The prior probability $\pi(z_{0}|y)$ is then calculated through the change of variable formula such as presented in the equation \ref{eq:conditional-change-of-variable-formula}.
    Concurrently,
        $z_{0}$ is also given as input to the decoder model,
        decoding $z_{0}$ back to $x$.
        
    The whole model described above is jointly trained using stochastic gradient descent with mini-batches.
    In this setting,
        the ELBO becomes:
        \input{content/cfvae/equations/eq_cfvae_elbo}
        where $\omega$, 
        $\phi$ 
        and $\theta$ are the model's trainable parameters.
    Thus,
        by passing the log-posterior expectation to the left side of equation \ref{eq:elbo-cfvae},
        we define a new lower-bound for the model optimization: 
        % the log evidence plus the log-posterior  expectation as follows:
        \input{content/cfvae/equations/eq_cfvae_lower_bound}%
    
    By optimizing the right side of equation \ref{eq:cfvae-lower-bound}, 
        we indirectly optimize its left side, 
        and therefore the loss function is written as follows:   
        \input{content/cfvae/equations/eq_cfvae_loss}%
    This loss function has two terms that,
        such as in VAEs,
        can be interpreted as the reconstruction error
        and the regularization terms. 
    The regularization term encourages the $z_{0}$ distribution to be close to the estimated prior distribution $\pi_{\omega}(z_{0}|y)$.
    It is calculated by the change of variable formula  
        presented in equation \ref{eq:conditional-change-of-variable-formula}.
    Since the decoder targets $x$ are in the continuous space,
        we consider that the decoder is 
        a multivariate Gaussian with a diagonal covariance structure.
    Thus, we use the usually chosen squared error simplification for the reconstruction error term.
    
    The generative process is done by 
        first sampling $z_{k}$ from a simple base density,
        such as a diagonal Gaussian distribution
        whose parameters are calculated by the conditioning network using the $y$ observation.
    The conditioning network also outputs a hidden state $h(y)$,
        which is passed as input to the inverse mapping together with $z_k$ to recover the latent variable $z_{0}$ such that $z_{0} = f^{-1}(z_{k}, h(y))$. 
    Thus,
        the conditioning network has three outputs
        $\mu(h(y))$, 
        $\sigma(h(y))$,
        and $h(y)$. 
    At last,
        $z_{0}$ is decoded by the generative model $q_{\phi}(x | z_{0}, h(y))$.

    Note that
        to maintain compatibility with the CVAE formulation,
       $h(y)$ is also passed as input to the generative model.
    % Therefore,
    %     the CFN inverse mapping becomes $z_{0} = f_{\omega}^{-1}(z_{k};h(y))$,
    %     and the generative model becomes $q_{\phi}(x | z_{0}, h(y))$.
        
    Figure \ref{fig:cfvae-train-and-inference-schemes}
        illustrates the model's training and inference schemes.
    In (a), 
        we present the training flow scheme, 
        where the outputs $\hat{x}$ 
        and $z_{k}$ are used to compute the loss function, 
        such as defined by equation \ref{eq:loss-elbo}.
    In (b), 
        we present the inference flow scheme, 
        where we use the conditioning network outputs,
        $\mu(h(y))$ and  $\sigma(h(y))$, 
        to sample $z_{k}$ through the reparametrization trick 
        and passing it through the CNF inverse pass pass to recover $z_{0}$.
    Note that,
        in both (a) and (b),
        we concatenate $z_0$ and $h(y)$ 
        into a single tensor before serving them as inputs to the decoder network, 
        but the inputs are not concatenated in the CNF.
    It is omitted from the diagrams for simplicity.
        % 
    \input{content/cfvae/figures/fig_cfvae_schemes}%

==> content/dataset/dataset.tex <==
\section{Dataset} \label{sec:dataset}

   
    
    

==> content/experiments/old/ablation.tex <==
\subsection*{Ablation Studies}  \label{sec:ablation}
    In the {\ModelName} architecture, we included two components that work for conditioning the generative process on the aggregate data $y$, which are (1) the $h(y)$ connections in the affine coupling layers and (2) the conditioning from $z_{k}$ base distribution in the CNF.
    Therefore, 
        to investigate these components' importance to the model, 
        we conducted two experiments consisting of training and testing {\ModelName}
        variations without each of these components. 
    
    In both experiments,
        the data and the model hyper-parameters were kept constant 
        while different {\ModelName} versions were evaluated.   
    The models were trained for six of the eight machines, 
        using $80\%$ of the dataset. 
    The remaining $20\%$ of the dataset was used for testing.
    Additionally,
        we present the total sum and the averaged metrics over the six machines
        \footnote{We present the individual results in the supplementary material. }.
    Thus,
        the metrics are computed individually for each machine, 
        and then the total sum and the average values are calculated.
    
    % We compared the performance of these two modified versions against the complete {\ModelName} model's.
    First,
        we compared the complete {\ModelName} model's performance against two modified versions.
    In the first modified version, 
        we removed the $h(y)$ connections 
        from the affine coupling layers 
        by exchanging them for its simple (and original) version.
    In the second modified version, 
        we removed the conditioning from the $z_{k}$ base distribution, 
        in the CNF, 
        by fixing its parameters to match the diagonal standard normal distribution such that $\pi(z_{k}|y) \sim \mathcal{N}(0,1)$. 
    As a consequence,
            we removed the 
            $\mu(h(y))$ and $\sigma(h(y))$ 
            calculations from the model.
        
    \input{content/experiments/tables/conditioning_ablations_table}
    
    Table \ref{tab:conditioning-ablations} compares the averaged and total resulting metrics of the 
    complete model, 
    the simple affine coupling layer,
    and the standard normal base distribution versions.
    
    The standard normal base distribution version results 
        were around ten times worse in both metrics than the other versions,
        which might indicate that 
        learning the base distribution parameters allows 
        the CNF to estimate tighter and more flexible distributions for $z_{0}$.
        
    % The comparison of the simple affine coupling layer version
    %     against the complete model indicates that 
    %     the capability of both versions in predicting the overall energy consumption 
    %     for the appliances is quite similar, 
    %     since the SAE for these two version are very close.
    Comparing the simple affine coupling layer version 
        against the complete model indicates that 
        both versions' capability in predicting the overall energy consumption 
        for the appliances is quite similar 
        since the SAE for these two versions is very close.
    However, 
        the significant difference in the NDE indicates that
        the complete model has a stronger capability
        to predict appliance instantaneous power demand.
    Therefore, 
        the usage of the $h(y)$ connections 
        in the affine coupling layers seem to be 
        necessary for the model's performance, 
        which justifies its use, 
        even though it increases the total number of parameters.
    
    Next, we performed another ablation study, 
        which consisted of
        analyzing the {\ModelName} model's performance 
        when varying the number of step-flow blocks used in the CNF.
    Table \ref{tab:cnf-ablations} compares 
        the averaged and total resulting metrics 
        for five trained model variants with 
        $2$, $4$, $8$, $16$, and $32$ 
        step-flow blocks in the CNF component.
        
    \input{content/experiments/tables/cnf_ablations_table}
    
    The model with $8$ step-flow blocks presented the best performance in both metrics. 
    It is worth noting that the performance improves by adding more blocks until $8$, 
        starting to degrade when adding more blocks, 
        as seen in the results for $16$ and $32$ blocks.
    It indicates that we must choose the number of step-flows sparingly 
        and that the model's performance degrades with very deep CNFs, 
        even though a too shallow model is not powerful enough to capture the latent space distribution. 
        
    In summary, 
        these experiments suggest that the best version of the {\ModelName} for the task is the one where the CNF is built with $8$ step-flow blocks, 
        uses learned features $h(y)$ in its affine coupling layers,
        and is conditioned on the $z_k$ base distribution.
    

==> content/experiments/old/cross_validation.tex <==
\subsection*{Cross-Validation}  \label{sec:results} 
    % The {\ModelName} performance was evaluated using two commonly used metrics in NILM tasks \cite{zhong2014signal}: 
    %     (1) the normalized disaggregation error (NDE) 
    %     and (2) the signal aggregated error (SAE). 
    % The NDE is used for verifying the capability of a NILM model in predicting the appliance's instantaneous power demand, 
    %     while the SAE, 
    %     in predicting the appliance's total energy consumption.
    
    % Those metrics are calculated from the average of $20$ samples taken with the trained model using the aggregated data $y$ as input.
    
    % Those metrics are obtained in a {\NFolds}-fold cross-validation setting \cite{CV:Kohavi:1995}.
    This experiment is performed in a {\NFolds}-fold cross-validation setting \cite{CV:Kohavi:1995}.
    The models are trained using the setup described in section \ref{sec:architecture} at each cross-validation iteration.
    The training procedure takes on average 17 hours per cross-validation iteration.
    % The whole experiment is performed in a {\NFolds}-fold cross-validation setting \cite{CV:Kohavi:1995},
        % where the {\ModelName} model is trained using the setup
        % described in section \ref{sec:architecture} at each iteration.
    % For performing the cross-validation,
    % Therefore,
    %     we split the dataset into {\NFoldsWritten} non-overlapping folds, 
    %     and then, 
    %     leaving one distinct fold out at a time, 
    %     we fit one {\ModelName} model with the remaining folds.
    % The left-out folds are used to compute the evaluation metrics for their respective model.
    % In all cross-validation iterations,
    %     the {\ModelName} model is trained using the setup
    %     described in section \ref{sec:experimental-setup}.%, 
        % for {\NEpochs} epochs.
    
    Additionally, 
        since the amount of available data for the milling machines (MI and MII) is much smaller than the available data for the other appliances,
        we perform the cross-validation apart for these machines.
    % Since the amount of available data for the milling machines (MI and MII) is much smaller than the available data  for the other appliances, 
    % we train a {\ModelName} model apart for these machines. 
    % one dedicated for performing the disaggregation task for the milling machines data and the other for the other 6 appliances. 
    
    Table \ref{tab:results} compares the obtained metrics with the WaveNet (WN) model, 
        proposed by the previous work \cite{Martins2018ApplicationOA} on the same dataset.
    
    \input{content/experiments/tables/results_table}
    
    The table shows that the {\ModelName} consistently improves the metrics in six of the eight machines belonging to the dataset.
    Analyzing the NDE metric, 
        the improvements go from {\PINDEImprovement}, 
        for the \textit{PI} machinery, 
        up to {\MINDEImprovement}, 
        for the \textit{MI} machinery.
    % Additionally, 
    %     we observe an error increase of 
    %     {\EFINDEIncrease} for the \textit{EFI} machinery 
    %     and {\EFIINDEIncrease} for the \textit{EFII} machinery.
    Additionally, 
        we observe an error increase for the \textit{EFI} and \textit{EFII} machinery.
    
    In it turns, 
        improvements in SAE go from {\PIISAEImprovement} 
        for the \textit{PII} machinery 
        up to {\DPCIISAEImprovement} for the \textit{DPCII} machinery.
    % Additionally, 
    %     we observe an error increase of {\EFISAEIncrease} for the \textit{EFI} machinery 
    %     and {\EFIISAEIncrease} for the \textit{EFII} machinery.
    Additionally, 
        we observe an error increase for the \textit{EFI},
        \textit{EFII}, and \textit{MII} machinery.
    
    Finally, the PFVAE's higher representational capacity enables the usage of all electrical quantities available in the dataset as input features that might explain the model's overall improvements.
    Moreover, 
        due to the factory's operation routine, 
        the appliance activations are generally related to each other. 
    Therefore learning to represent multiple appliance activations using a single model can be beneficial.
    % We enumerate the two main reasons reasons that might explain the overall improved results when using the PFVAE model:
    
    % \begin{enumerate}
    %     \item the model's higher capacity of representation enables the usage of all of the electrical quantities available in the dataset as its features;
    %     \item due to the factory's operation routine, the appliances activations are genereally related to each other, therefore learning to represent multiple appliances activations using a single model can be beneficial.
    % \end{enumerate}
    
    

==> supplementary_material/abstract.tex <==
\begin{abstract}
    
    This document provides supplementary material for the paper entitled 
        -- 
        Prior Flow Variational Autoencoder: 
        A density estimation model for Non-Intrusive Load Monitoring.
    In the following, 
        we provide more detailed information about the results reported in the paper, 
        including per machinery comparison tables for the ablation studies 
        and comparisons of the models' optimization curves for each ablation.
    Additionally,  
        we present visual comparison plots between 
        the ground truth data 
        and the model predictions.
\end{abstract}

==> supplementary_material/experiments/tables/results_table.tex <==
% \newcolumntype{R}{>{\raggedleft\arraybackslash}X}%
% \newcolumntype{L}[1]{>{\raggedright\arraybackslash}X}%
\begin{table}[ht]
    \caption{
        Performance comparison between the {\ModelName} and the Wavenet (WN) models.
    }
    \label{tab:results}
    \begin{center}
    \begin{small}
    \begin{sc}
    \begin{tabularx}{0.8\columnwidth}{X ll}
        &
            \multicolumn{2}{c}{NDE} \\
        &  
             \multicolumn{1}{c}{WN} 
            %  WN 
        & 
            \multicolumn{1}{c}{{\ModelName}} \\   
            % {\ModelName} \\   
        \bottomrule
        \midrule
        
        PI    & 
            0.045 $\pm$ 0.002  &  {\ndePI} \\
            
        PII    & 
            0.056 $\pm$ 0.002 & {\ndePII} \\
                
        DPCI    & 
            0.08 $\pm$ 0.01  & {\ndeDPCI} \\
        
        DPCII    & 
            0.202 $\pm$ 0.006  & {\ndeDPCII} \\
        
        EFI    & 
            \textbf{0.046 $\pm$ 0.0004}  & {\ndeEFI} \\
            
        EFII    & 
            \textbf{0.041 $\pm$ 0.003}  & {\ndeEFII} \\
            
        MI    & 
            0.08 $\pm$ 0.02  & {\ndeMI} \\
        
        MII    & 
            0.06 $\pm$ 0.01  & {\ndeMII} \\
        \\    
        % \midrule 
        % \toprule
        &
            \multicolumn{2}{c}{SAE} \\
        &  
             \multicolumn{1}{c}{WN}
        & 
            \multicolumn{1}{c}{{\ModelName}} \\
        \bottomrule   
        \midrule
        
        PI    & 
            0.047 $\pm$ 0.009 & {\saePI} \\
            
        
        PII    & 
            0.022 $\pm$ 0.009 & {\saePII} \\
                
        DPCI    & 
            0.13 $\pm$ 0.04  & {\saeDPCI} \\
        
        DPCII    & 
            0.19 $\pm$ 0.02  & {\saeDPCII} \\
        
        EFI    & 
            \textbf{0.007 $\pm$ 0.006}  & {\saeEFI} \\
            
        EFII    & 
            \textbf{0.016 $\pm$ 0.009}  & {\saeEFII} \\ 
            
        MI    & 
            0.09 $\pm$ 0.04 & {\saeMI} \\
            
        MII    & 
            \textbf{0.03 $\pm$ 0.02} & {\saeMII} %\\
            
    \end{tabularx}
    \end{sc}
    \end{small}
    \end{center}
    \vskip -0.15in
\end{table}

